Budgeted Dominating Sets in Uncertain Graphs

We study the {\em Budgeted Dominating Set} (BDS) problem on uncertain graphs, namely, graphs with a probability distribution $p$ associated with the edges, such that an edge $e$ exists in the graph with probability $p(e)$. The input to the problem consists of a vertex-weighted uncertain graph $\G=(V, E, p, \omega)$ and an integer {\em budget} (or {\em solution size}) $k$, and the objective is to compute a vertex set $S$ of size $k$ that maximizes the expected total domination (or total weight) of vertices in the closed neighborhood of $S$. We refer to the problem as the {\em Probabilistic Budgeted Dominating Set}~(PBDS) problem and present the following results. \begin{enumerate} \dnsitem We show that the PBDS problem is NP-complete even when restricted to uncertain {\em trees} of diameter at most four. This is in sharp contrast with the well-known fact that the BDS problem is solvable in polynomial time in trees. We further show that PBDS is \wone-hard for the budget parameter $k$, and under the {\em Exponential time hypothesis} it cannot be solved in $n^{o(k)}$ time. \item We show that if one is willing to settle for $(1-\epsilon)$ approximation, then there exists a PTAS for PBDS on trees. Moreover, for the scenario of uniform edge-probabilities, the problem can be solved optimally in polynomial time. \item We consider the parameterized complexity of the PBDS problem, and show that Uni-PBDS (where all edge probabilities are identical) is \wone-hard for the parameter pathwidth. On the other hand, we show that it is FPT in the combined parameters of the budget $k$ and the treewidth. \item Finally, we extend some of our parameterized results to planar and apex-minor-free graphs. \end{enumerate}

==> comments.tex <==
we need to state given any instance of partition problem K can be scaled to meet our constraint.

1. inconsistency of \Ohk() and O()
2. w is already used to denote treewidth, so need to ensure that weight is represented as "wt" throughout the paper.

==> figure/gadget2.tex <==
\begin{figure}[h]
\center
\begin{tikzpicture}
\makeatletter
\tikzset{
    dot diameter/.store in=\dot@diameter,
    dot diameter=3pt,
    dot spacing/.store in=\dot@spacing,
    dot spacing=10pt,
    dots/.style={
        line width=\dot@diameter,
        line cap=round,
        dash pattern=on 0pt off \dot@spacing
    }
}
\makeatother
\coordinate (v) at (1,0);
\coordinate (a) at (-4, -2);
\coordinate (b) at (-2, -2);
\coordinate (c) at (0, -2);
\coordinate (d) at (6, -2);

\draw[black, thick] (v) -- (a) node[midway, left] {$p_1$};
\draw[black, thick] (v) -- (b) node[midway, right] {$p_2$};
\draw[black, thick] (v) -- (c) node[midway, right] {$p_3$};
\draw[black, thick] (v) -- (d) node[midway, right] {$p_n$};

\draw[black, thick] (a) -- ($(a) + (-0.75,-2)$) node[midway, left] {$1.0$};
\draw[black, thick] (b) -- ($(b) + (-0.75,-2)$) node[midway, left] {$1.0$};
\draw[black, thick] (c) -- ($(c) + (-0.75,-2)$) node[midway, left] {$1.0$};
\draw[black, thick] (d) -- ($(d) + (-0.75,-2)$) node[midway, left] {$1.0$};

\draw[black, thick] (a) -- ($(a) + (0.75,-2)$) node[midway, left] {$1.0$};
\draw[black, thick] (b) -- ($(b) + (0.75,-2)$) node[midway, left] {$1.0$};
\draw[black, thick] (c) -- ($(c) + (0.75,-2)$) node[midway, left] {$1.0$};
\draw[black, thick] (d) -- ($(d) + (0.75,-2)$) node[midway, left] {$1.0$};

\fill[white] (v) circle (0.15cm);
\draw[black, thick] (v) circle (0.15cm) node[right=0.15cm] {$v_0$};

\fill[white] (a) circle (0.15cm);
\draw[black, thick] (a) circle (0.15cm) node[left=0.15cm] {$v_1$};
\fill[white] (b) circle (0.15cm);
\draw[black, thick] (b) circle (0.15cm) node[left=0.15cm] {$v_2$};
\fill[white] (c) circle (0.15cm);
\draw[black, thick] (c) circle (0.15cm) node[left=0.15cm] {$v_3$};
\fill[white] (d) circle (0.15cm);
\draw[black, thick] (d) circle (0.15cm) node[left=0.15cm] {$v_n$};

\draw [black, dot diameter=3pt, dot spacing=10pt, dots] ($(c) + (1.5, 0)$) -- ($(d) + (-1.5, 0)$);

\fill[white] ($(a) + (0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(a) + (0.75,-2)$) circle (0.15cm) node[below=0.15cm] {$v_{2n+1}$};
\fill[white] ($(b) + (0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(b) + (0.75,-2)$) circle (0.15cm) node[below=0.15cm] {$v_{2n+2}$};
\fill[white] ($(c) + (0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(c) + (0.75,-2)$) circle (0.15cm) node[below=0.15cm] {$v_{2n+3}$};
\fill[white] ($(d) + (0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(d) + (0.75,-2)$) circle (0.15cm) node[below=0.15cm] {$v_{3n}$};

\fill[white] ($(a) + (-0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(a) + (-0.75,-2)$) circle (0.15cm) node[right=0.1cm] {$v_{n+1}$};
\fill[white] ($(b) + (-0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(b) + (-0.75,-2)$) circle (0.15cm) node[right=0.1cm] {$v_{n+2}$};
\fill[white] ($(c) + (-0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(c) + (-0.75,-2)$) circle (0.15cm) node[right=0.1cm] {$v_{n+3}$};
\fill[white] ($(d) + (-0.75,-2)$) circle (0.15cm);
\draw[black, thick] ($(d) + (-0.75,-2)$) circle (0.15cm) node[right=0.1cm] {$v_{2n}$};
\end{tikzpicture}
\caption{}
\label{fig:localStructure}
\end{figure}

==> figure/treeReduction.tex <==
\begin{figure}
\begin{tikzpicture}
\coordinate (a) at (0,1);
\coordinate (b) at ($(a) + (2.5,-1)$);
\coordinate (c) at ($(b) + (3,1)$);
\coordinate (d) at ($(c) + (3,-1)$);

\draw[black] ($(a)+(0.75,1)$) -- ($(a)+(0.75,0)$);
\draw[black] ($(a)+(0.75,1)$) -- (a);
\draw[black] ($(a)+(0.75,1)$) -- ($(a)+(1.5,0)$);
\draw[black, dashed] ($(a)+(0.75,1)$) -- ($(a)+(1.5,2)$);
\fill[white] (a) circle (0.15);
\fill[white] ($(a)+(0.75,0)$) circle (0.15);
\fill[white] ($(a)+(1.5,0)$) circle (0.15);
\fill[white] ($(a)+(0.75,1)$) circle (0.15);
\fill[white] ($(a)+(1.5,2)$) circle (0.15);
\draw[black] (a) circle (0.15) node {$b$};
\draw[black] ($(a)+(0.75,0)$) circle (0.15) node {$c$};
\draw[black] ($(a)+(1.5,0)$) circle (0.15) node {$d$};
\draw[black] ($(a)+(0.75,1)$) circle (0.15) node {$a$};
\draw[black] ($(a)+(1.5,2)$) circle (0.15) node {$p$};

\draw[black, ->, ultra thick] ($(a)+(1.75,1)$) -- ($(a)+(3,1)$);
        
\draw[black] ($(b)+(0.5,1)$) -- ($(b)+(1,2)$);
\draw[black] ($(b)+(0.5,1)$) -- (b);
\draw[black] ($(b)+(0.5,1)$) -- ($(b)+(1,0)$);
\draw[black] ($(b)+(1,2)$) -- ($(b)+(1.5,1)$);
\draw[black, dashed] ($(b)+(1,2)$) -- ($(b)+(1.5,3)$);
\fill[white] (b) circle (0.15);
\fill[white] ($(b)+(1,0)$) circle (0.15);
\fill[white, gray] ($(b)+(0.5,1)$) circle (0.15);
\fill[white] ($(b)+(1.5,1)$) circle (0.15);
\fill[white] ($(b)+(1,2)$) circle (0.15);
\fill[white] ($(b)+(1.5,3)$) circle (0.15);
\draw[black] (b) circle (0.15) node {$b$};
\draw[black] ($(b)+(1,0)$) circle (0.15) node {$c$};
\draw[gray] ($(b)+(0.5,1)$) circle (0.15) node[black, left=0.15cm] {$q_1$};
\draw[black] ($(b)+(1.5,1)$) circle (0.15) node {$d$};
\draw[black] ($(b)+(1,2)$) circle (0.15) node {$a$};
\draw[black] ($(b)+(1.5,3)$) circle (0.15) node {$p$};

\draw[black] ($(c)+(1.125,1)$) -- (c);
\draw[black] ($(c)+(1.125,1)$) -- ($(c)+(0.75,0)$);
\draw[black] ($(c)+(1.125,1)$) -- ($(c)+(1.5,0)$);
\draw[black] ($(c)+(1.125,1)$) -- ($(c)+(2.25,0)$);
\draw[black, dashed] ($(c)+(1.125,1)$) -- ($(c)+(1.75,2)$);
\fill[white] (c) circle (0.15) ;
\fill[white] ($(c)+(0.75,0)$) circle (0.15) node {$d$};
\fill[white] ($(c)+(1.5,0)$) circle (0.15) node {$e$};
\fill[white] ($(c)+(2.25,0)$) circle (0.15) node {$f$};
\fill[white] ($(c)+(1.125,1)$) circle (0.15) node {$a$};
\fill[white] ($(c)+(1.75,2)$) circle (0.15) node {$p$};
\draw[black] (c) circle (0.15) node {$b$};
\draw[black] ($(c)+(0.75,0)$) circle (0.15) node {$d$};
\draw[black] ($(c)+(1.5,0)$) circle (0.15) node {$e$};
\draw[black] ($(c)+(2.25,0)$) circle (0.15) node {$f$};
\draw[black] ($(c)+(1.125,1)$) circle (0.15) node {$a$};
\draw[black] ($(c)+(1.75,2)$) circle (0.15) node {$p$};

\draw[black, ->, ultra thick] ($(c)+(2.25,1)$) -- ($(c)+(3.75,1)$);

\draw[black] ($(d)+(0.5,1)$) -- (d);
\draw[black] ($(d)+(0.5,1)$) -- ($(d)+(1,0)$);
\draw[black] ($(d)+(0.5,1)$) -- ($(d)+(1.5,2)$);
\draw[black] ($(d)+(2.5,1)$) -- ($(d)+(1.5,2)$);
\draw[black] ($(d)+(2.5,1)$) -- ($(d)+(2,0)$);
\draw[black] ($(d)+(2.5,1)$) -- ($(d)+(3,0)$);
\draw[black] ($(d)+(1.5,2)$) -- ($(d)+(2,3)$);
\fill[white] (d) circle (0.15) node {$b$};
\fill[white] ($(d)+(1,0)$) circle (0.15) node {$c$};
\fill[white] ($(d)+(2,0)$) circle (0.15) node {$d$};
\fill[white] ($(d)+(3,0)$) circle (0.15) node {$e$};
\fill[gray] ($(d)+(0.5,1)$) circle (0.15) node[black, left=0.15cm] {$q_1$};
\fill[gray] ($(d)+(2.5,1)$) circle (0.15) node[black, right=0.15cm] {$q_2$};
\fill[white] ($(d)+(1.5,2)$) circle (0.15) node {$a$};
\fill[white] ($(d)+(2,3)$) circle (0.15) node {$p$};
\draw[black] (d) circle (0.15) node {$b$};
\draw[black] ($(d)+(1,0)$) circle (0.15) node {$c$};
\draw[black] ($(d)+(2,0)$) circle (0.15) node {$d$};
\draw[black] ($(d)+(3,0)$) circle (0.15) node {$e$};
\draw[gray] ($(d)+(0.5,1)$) circle (0.15) node[black, left=0.15cm] {$q_1$};
\draw[gray] ($(d)+(2.5,1)$) circle (0.15) node[black, right=0.15cm] {$q_2$};
\draw[black] ($(d)+(1.5,2)$) circle (0.15) node {$a$};
\draw[black] ($(d)+(2,3)$) circle (0.15) node {$p$};
\end{tikzpicture}
\caption{Gadgets for the higher degree nodes.}
\end{figure}

==> fpt-treewidth.tex <==
\section{Fixed Parameter Tractable Algorithms}
\label{section:fpt}
\subsection{Solving PBDS on Bounded-Treewidth graphs} 

%We give a dynamic programming algorithm working on a so-called \emph{nice tree decomposition} of the input graph $\G$.
%In this subsection, we prove the following theorem. %Theorem~\ref{theorem:fpt-by-wk}.

%\begin{theorem}\label{theorem:fpt-by-wk}
%For any integer $k$, and any $n$-vertex weighted graph $G$ with arbitrary edge survival probabilities and treewidth $w$, we can compute a $(1-\epsilon)$-approximation to the optimal \pkbds in $((1/\epsilon)2^{\Oh(w \log k)}n^3)$ time.
%
%Moreover, if the edge survival probabilities in $G$ are identical then our algorithm solves the problem exactly in $(2^{\Oh(w \log k)}n^3)$ time.
%\keerti{It might be better to state the exact time complexity (that would be probably just linear in $n$)}
%\end{theorem}
\noindent
We assume that a nice tree decomposition $(\TD, X)$ rooted at $\blr$ is given
(See Appendix~\ref{apdx:sec:twdefinition} for treewidth-related definitions).
Consider the following dynamic program (DP) on $(\TD,X)$.
Given a node $\bli \in V(\TD)$, a state for the node $\bli$ is a tuple
$(b, c, \alpha, \beta)$, where
(a) $0 \leq b \leq k$ is the solution size to be computed,
(b) $c:\Xi\to \{0,1\}$ is an indicator function where $c(u)=1$
if $u$ is included in the solution,
(c) $\alpha:\Xi\to [0,k]$
%is a function indicating
gives, for each vertex $u\in\Xi$,
the number $\alpha(u)$ of neighbors from $\Xi^+$ that must be in the solution,
and (d) $\beta:\Xi \to [0,k]$
%is a function indicating
gives, for each vertex $u\in\Xi$,
the number $\beta(u)$ of neighbors of $u$ from $V\setminus \Xi^+$ that will be
added to the solution at a later state of the exectuion.
%Note that the later state would be at an accestor of node $\bli$.
Let $\S_\bli$ be the set of all $\Oh(k^w)$ states associated with node $\bli$.
We now define the solution functions $\sol_\bli : \S_\bli \to 2^V$ and
$\val_\bli : \S_\bli \to \mathbb{Q}$.
For a state $s = (b,c,\ca,\cb)$, 
consdier the Uni-PBDS problem on instance $\G$ with budget $b$ and
vertex weight function $\wt^s:\Xi^+ \to \mathbb{R}$,
%$\wt^s $\langle \G[\Xi^+], \wt^s, b\rangle$ is considered where $\wt^s$ is
%where the weight function $\wt^s:\Xi^+ \to \mathbb{R}$ 
defined as follows. For each vertex $u \in \Xi^+$,
\[\wt^s_u = \begin{cases}
\big((1-p)^{\cb(u)}\big)\wt_u, & \text{ if } u \in \Xi \text{ and } c(u) = 0,\\
\wt_u, & \text{ if } u \in \Xi \text{ and } c(u) = 1,\\
\wt_u, & \text{ if } u \notin \Xi.
\end{cases}\]
The set $\soli$ is an optimal feasible solution to this instance.
In other words, it is a solution that satisfies
$(a)$ $|\soli| = b$ and $\soli \cap \Xi = c\inv(1)$, $(b)$ For each $u \in \Xi$ with $c(u) = 0$, $|N(u) \cap \Xi^+ \cap \soli| = \ca(u)$, and $(c)$ $\vali(s) = \C(V, \soli(s))$. 
The state $s = (b,c,\ca,\cb)$ is said to be \emph{invalid} if no feasible solution exists.
The DP computes the functions $\soli$ and $\vali$ for each node $\bli \in V(\TD)$.
Note that for the root $X_\blr = \emptyset$, the state set $\S_\blr$ is a singleton with a state $s = (k, \emptyset\to\{0,1\}, \emptyset\to[0,k], \emptyset \to [0,k])$.
$\sol_\blr(s)$ is an optimal solution for the Uni-PBDS problem on instance $\langle \G, k \rangle$.
The DP uses four types of nodes, called leaf nodes, introduce nodes,
forget nodes and join nodes, whose corresponding update steps are presented in
Appendix~\ref{apdx:sec:dp}. From the description in the appendix, it follows
that the values for each state can be computed in time $\Oh(k^{w}n^2)$.
Thus, an optimal solution can be computed in time $2^{\Oh(w \log k)}n^3$.

\begin{theorem}\label{theorem:fpt-by-wk}
The Uni-PBDS problem can be solved in time $2^{\Oh(w \log k)}n^3$ where $w$ is the treewidth of the input graph.
\end{theorem}

%We describe our dynamic program in cases according to the types of nodes of the nice tree decomposition.
%Due to Lack in space,
%	\noindent {\bf Leaf node}: Let $\bli$ be a leaf node with bag $\Xi = \emptyset$. The state set $\S_\bli$ is a singleton with a state $s = (0, \emptyset\to\{0,1\}, \emptyset\to[k], \emptyset \to [k])$. Then,
%	$\soli(s) = \emptyset \text{ and } \vali(s) = 0.$
%	This can be calculated in constant time.
%	For the correctness, note that the graph $\G[\Xi^+]$ is a \emph{null graph}.
%	
%	\noindent {\bf Introduce node}: Let $\bli$ be an introduce node with a child $\blj$ such that $\Xi = \Xj \cup \{v\}$ for some $v \notin \Xj$.
%	Recall that $v$ is referred to as an introduced vertex.
%	Let $C_v = N(v) \cap \Xi$.
%	Consider a state $s =(b,c,\ca,\cb) \in \Si$ and a state $s' = (b',c',\ca',\cb') \in \Sj$.
%	We say that $s'$ is consistent with $s$, or $s' \preceq s$ if one of the following is satisfied:
%	\begin{itemize}
%	\item[(i)] If $c(v)=1$ then $b=b'+1$, and for each vertex $u \in \Xj$, $c(u) = c'(u)$, and if $u \in C_v$ then $\ca(u) = \ca'(u) + 1$ and $\cb(u) = \cb'(u) - 1$, otherwise $\ca(u) = \ca'(u)$ and $\cb(u) = \cb'(u)$.
%	%\begin{itemize}
%	%\item $b = b' + 1$,
%	%\item for each vertex $u \in \Xj$, $c(u ) = c'(u)$,
%	%\item for each vertex $u \in \big(\Xi \cap C_v\big)$, $\ca(u) = \ca'(u) + 1$ and $\cb(u) = \cb'(u)-1$, and
%	%\item for each vertex $u \in \big(\Xi\setminus C_v\big)$, $\ca(u) = \ca'(u)$ and $\cb(u) = \cb'(u)$.
%	%\end{itemize}
%	\item[(ii)] If $c(v) = 0$ then $b = b'$ and for each vertex $u \in \Xj$, $c(u ) = c'(u)$,  $\ca(u) = \ca'(u)$ and $\cb(u) = \cb'(u)$.
%	%\begin{itemize}
%	%\item $b = b'$ and
%	%\item for each vertex $u \in \Xj$, $c(u ) = c'(u)$,  $\ca(u) = \ca'(u)$ and $\cb(u) = \cb'(u)$.
%	%\end{itemize}
%	\end{itemize}
%	Note that for each state $s \in \Si$, there is an unique state $s' \in \Sj$ such that $s' \preceq s$.
%	If $c(v) = 0$ and $|C_v| \not= \ca(v)$ then the state $s$ has no feasible solution. Thus, we assume the cases either $c(v) = 1$, or $c(v) = 0$ and $|C_v| = \ca(v)$.
%	Therefore,
%	\begin{equation}
%	\soli(s) = \begin{cases}
%	\solj(s') & \text{ if } c(v) = 0, \\
%	\solj(s') \cup \{v\} & \text{ otherwise}
%	\end{cases}
%	\end{equation}
%	and
%	\begin{equation}
%	\label{eqn:dpinval}
%	\vali(s) = \begin{cases}
%	\valj(s')+\big( 1- (1-p)^{\ca(v)} \big)\wt^s_v & \text{ if } c(v) = 0, \\
%	\valj(s')+\wt^s_v + \displaystyle\sum_{u \in C_v \mid c(u) = 0} p\ \wt^s_u & \text{ otherwise}.
%	\end{cases}
%	\end{equation}
%	This can be calculated in $\Oh(w)$ time.
%	We prove the correctness as follows.
%	Let $\soli(s) = S \subseteq \Xi^+$. % and $\vali = t$ be the coverage value.
%	By definition of consistency, if $c(v) = 0$ then the solution $S$ is a feasible solution to the state $s'$ in node $\blj$, otherwise the solution $S\setminus \{v\}$ is a feasible solution to the state $s'$ in node $\blj$.
%	Conversely, the solution $\solj(s')$ is a feasible solution for the state $s$ in node $\bli$ when $c(v) = 0$, and the solution $\solj(s') \cup \{v\}$ is a feasible solution when $c(v) = 1$.
%	The above statements imply that an optimal solution for the state $s'$ in node $\blj$ gives an optimal solution for the state $s$ in node $\bli$.
%	The coverage values of the solutions in the two states differ only by contribution of $v$ when $c(v) = 0$, and by contribution of $v$ and $C_v$ when $c(v) = 1$.
%	In Equation~\ref{eqn:dpinval}, value $\vali(s)$ is calculated by adding appropriate additional coverage due to $v$.
%	Hence, our recurrence correctly computes the solution for the state $s$.
%	
%	\noindent {\bf Forget node}: Let $\bli$ be a forget node with child $\blj$ such that $\Xi = \Xj \setminus \{v\}$ for some $v \in \Xj$.
%	Recall that the vertex $v$ is referred as forgotten vertex.
%	Let $C_v = N(v) \cap \Xi$.
%	Consider a state $s =(b,c,\ca,\cb) \in \Si$ and a state $s' = (b',c',\ca',\cb') \in \Sj$.
%	We say that $s'$ is consistent with $s$, or $s' \preceq s$ if $b' = b$ and for each vertex $u \in \Xi$, $c(u) = c'(u)$, $\ca(u) = \ca'(u)$ and $\cb(u) = \cb'(u)$.
%	Note that there is no constraint over $v$ for $s'$ to be consistent with $s$.
%	Then, $v$ can have all possible values for the functions $c', \ca'$ and $\cb'$.
%	Thus, a state $s \in \Si$ can have at most $k^2$ consistent states in $\Sj$.
%	Let $\cons(\blj, s) = \{s' \in \Sj \mid s' \preceq s\}$.
%	Let $\hat{s} = \argmax_{s' \in \cons(\blj, s)} \valj(s')$.
%	Then,
%	\begin{equation}
%	\soli(s) = \solj(\hat{s})
%	\end{equation}
%	and
%	\begin{equation}
%	\label{eqn:dpfnval}
%	\vali(s) = \valj(\hat{s})
%	\end{equation}
%	This can be computed in $\Oh(w k)$ time.
%	We prove the correctness as follows.
%	Let $\soli = S \subseteq \Xi^+$. % and $\vali = t$.
%	Since $\Xi^+ = \Xj^+$, the solution $S$ is a feasible solution for the state $s'$. %$s' \in \cons(\blj, s)$.
%	By definition of consistency, an optimal solution to the state $s'$ in node $\blj$ is an optimal solution for the state $s$ in node $\bli$.
%	Then our recurrence correctly computes the solution for the state $s$.

%\noindent {\bf Join node}: Let $\bli$ be a join node with children $\blj$ and $\blh$ such that $\Xi = \Xj = \Xh$.
%Consider the following states $s = (b,c,\ca,\cb) \in \Si$, $s' = (b',c',\ca', \cb') \in \Sj$ and $s'' = (b'', c'', \ca'', \cb'') \in \Sh$.
%We say that the pair $(s',s'')$ is consistent with $s$, or $(s',s'') \preceq s$ if $b = b' + b'' - |c\inv(1)|$ and $\max(b',b'') \leq b$, and for each vertex $u \in \Xi$,  \begin{itemize}
%\item $c(u) = c'(u) = c''(u)$,
%\item $\ca(u) = \ca'(u) + \ca''(u) - |N(u) \cap c\inv(1)|$, and
%\item $\ca(u)+\cb(u) = \ca'(u) + \cb'(u) = \ca''(u) + \cb''(u)$.
%\end{itemize}
%%Intuitively, for each vertex $u \in \Xi$, $\ca'(u)$ and $\ca''(u)$ decompose $\ca(u)$ into two parts such that the neighbors in the bag are continuing as neighbors in states $s'$ and $s''$, and the additional neighbors are
%Let $s= (b,c,\ca,\cb) \in \Si$ be a state.
%Let $S \subseteq \Xi^+$ be an optimal solution for the state $s$.
%Let $\bar{S} = S \cap (\Xi^+\setminus \Xi)$.
%The set $\bar{S}$ can be partitioned into $\bar{S}_{\blj} \cup \bar{S}_{\blh}$ such that $\bar{S}_{\blj} = \bar{S} \cap (\Xj^+\setminus \Xj)$ and $\bar{S}_{\blh} = \bar{S} \cap (\Xh^+ \setminus \Xh)$ since $(\Xi^+ \setminus \Xi)= (\Xj^+\setminus \Xj) \uplus (\Xh^+\setminus \Xh)$.
%Then there exists a partition $b_{\blj}+b_{\blh} = b-|c\inv(1)|$ such that $b_{\blj} = |\bar{S}_{\blj}|$ and $b_{\blh} = |\bar{S}_{\blh}|$.
%Let $u\in c\inv(0)$ be a vertex and $C_u = N(v) \cap \Xi \cap c\inv(1)$.
%We know that $|C_u| \leq \ca(u)$, otherwise the state $s$ is invalid.
%Then, $\ca(u)-|C_u|$ vertices in $\bar{S}$ should cover $u$ and let $\bar{S}_{\bli, u} = N(u) \cap \bar{S}$ be such a set.
%The set $\bar{S}_{\bli, u}$ can be partitioned into $\bar{S}_{\blj,u} \cup \bar{S}_{\blh,u}$ such that $\bar{S}_{\blj,u} = \bar{S}_{\bli,u} \cap (\Xj^+\setminus \Xj)$ and $\bar{S}_{\blh,u} = \bar{S}_{\bli,u} \cap (\Xh^+\setminus \Xh)$.
%Then, there exists a partition $x+y = \ca(u) - |C_u|$ such that $x = |\bar{S}_{\blj,u}|$ and $y =|\bar{S}_{\blh,u}|$.
%Given a partition $b_{\blj}+b_{\blh} = b-|c\inv(1)|$, and a partition $x+y = \ca(u) - |C_u|$ for each vertex $u \in c\inv(0)$, there exists a pair of states $s' = (b',c',\ca',\cb') \in \Sj$ and $s''=(b'',c'',\ca'',\cb'') \in \Sh$ such that $b' = b_{\blj}$, $b'' = b_{\blh}$ and for each vertex $u\in \Xi$, $c'(u) = c''(u) = c(u)$, $\ca'(u) = x$, $\ca''(u) = y$.
%Thus each such partition defined above induces a consistent pair $(s',s'')$ for the state $s$ and there exists a consistent pair such that the solutions of the states will give solution for the state $s$.
%
%We now compute an optimal consistent pair for the state $s$.
%The different possible values of $b'$ and $b''$ are at most $b+1$.
%For each vertex $u \in \Xi$, $c'(u)$ and $c''(u)$ are fixed but $\ca'(u), \ca''(u), \cb'(u)$ and $\cb''(u)$ will have all possible values. %will get at most $(k+1)^2$ possible  values.
%Then, the state $s$ will have at most $(b+1)(k+1)^{2w} = \Oh(k^{2w+1})$ consistent pairs of states.
%Let $\cons(\blj, \blh, s) = \{(s', s'') \in \Sj\times\Sh) \mid (s', s'') \preceq s)\}$.
%We assume that for a fixed $(s',s'') \in \cons(\blj,\blh,s)$, the value $b'$ and $b''$, and the functions $c',c'',\ca',\ca'', \cb'$ and $\cb''$ are well defined.
%For a consistent pair $(s',s'') \in \cons(\blj,\blh,s)$ and a vertex $u \in c\inv(0)$, let us define
%\begin{equation*}
%\cd(s',s'',u) = \big( (1-p)^{\ca(u)-\ca'(u)} + (1-p)^{\ca(u) - \ca''(u)} - (1-p)^{\ca(u)}-1) \big)\wt^s_u.
%\end{equation*}
%The value $\lambda(s',s'',u)$ computes the over counting in coverage of $u$.
%Let
%\begin{equation*}
%s_\blj,s_\blh = \argmax_{(s',s'') \in \cons(\blj,\blh,s)} \Big(\valj(s') + \valh(s'')-\sum_{u\in c\inv(0)} \lambda(s',s'',u)\Big)
%\end{equation*}
%be an optimal consistent pair for $s$ in $\cons(\blj, \blh, s)$.
%Then,
%\begin{eqnarray*}
%\soli(s) &=& \solj(s_\blj) \cup \solh(s_\blh) \\
%\vali(s) &=& \valj(s_\blj) + \valh(s_\blh) - \sum_{u \in c\inv(0)} \lambda(s',s'',u)-\sum_{u \in c\inv(1)}\wt^s_u
%\end{eqnarray*}
%
%%The set $\cons(\blj,\blh,s)$ can be computed in $\Oh(wn)$%
%%\avi{Why do we need $\Oh(wn)$ time to compute $\cons(\blj,\blh,s)$? Can't we go over each of the  $k^{2w+1}$ combinations of $b'$ and $b''$, and the functions $\ca',\ca'', \cb'$ and $\cb''$ and compute the value $\cd(s',s'',u)$ in $\Oh(w)$? and then shouldn't the optimal consistent pair be computed in $\Oh(wk^{2w+1})$ time?}.
%An optimal consistent pair $(s_{\blj},s_{\blh})$ can be computed in $\Oh(w(k+1)^{2w+3}n^2)$ time.
%We prove the correctness as follows.
%We show that an optimal solution of the state can be obtained from the optimal solutions of the states in an optimal consistent pair.
%Then our recurrence correctly computes the solution for the state $s$.


==> treewidth.tex <==
%\section{Fixed Parameter Tractable Algorithms}
%\section{Paramterization based on graph structure}
%\label{section:fpt}
%%In this section, we present the algorithmic results obtained for the Uni-PBDS problem for different graph classes.
%In this section, we deal with structural parameterizations of the Uni-PBDS problem. % with its structural 
%First, we show that the Uni-PBDS is \wone-hard with respect to the parameter pathwidth of the input uncertain graph. 
%Then, we present an FPT algorithm for the Uni-PBDS problem parameterized by budget and the treewidth of the input graph.
%In addition, we show that the Uni-PBDS problem is FPT for the parameter budget on apex-minor-free graphs.
%On the algorithmic side, we have the following theorems.
%\begin{theorem}\label{theorem:fpt-by-wk}
%The {\sc PBDS} problem parameterized by $k$ and treewidth $w$ admits a $2^{\Oh(w \log k)}n^{\Oh(1)}$ time algorithm.
%\end{theorem}

%\begin{theorem}\label{theorem:fpt-amfg}
%The {\sc PBDS} problem admits an FPT algorithm on apex-minor-free graphs.
%\end{theorem
%In the remaining of this section, we will prove the two theorems stated above.

\subsection{Parameterization by treewidth and budget}
\label{sec:fptbtwg}

%Even if we applied many FPT tools to come up with an FPT algorithm parameterized by the solution size, we hit the bottle-neck of $\Delta$-factor on all our tries.

We present an algorithm for Uni-PBDS by dynamic programming
%algorithm to solve the Uni-PBDS. % and leave the details in Appendix~\ref{apdx:sec:dp}.
 on a nice tree decomposition 
 %\footnote{The definition of a nice tree decomposition is given in Appendix~\ref{apdx:sec:twdefinition}}
  of the input uncertain graph $\G$.\\
  
  \noindent
  {\bf Definitions and Notation}. We now set up the definitions and notation required for the DP formulation.
Let $(\TD, X)$ be a nice tree decomposition of the graph $\G$ rooted at node $\blr$. % is given to us.
For a node $\bli\in V(\TD)$, let $\TD_\bli$ be the subtree rooted at $\bli$ and
$\Xi^+ = \cup_{\blj \in  V(\TD_\bli)}\{\Xj\}$. 
The uncertain graph induced by the vertices $\Xi^+$ is $\G[\Xi^+]$ and it is denoted by $\Gi$.  
The expected domination function $\C$ over the graph $\Gi$ is denoted by $\Ci$.  We refer to the expected domination as coverage in the presentation below.
%Basically $\Gi$ denotes an instance 
%of Uni-PBDS. {\bf The edge weights must be clearly stated}

For each node $\bli \in \TD$, we compute two tables $\soli$ and $\vali$. 
The rows of both tables are indexed by 4-tuples which we refer to as states. $\S_\bli$ denotes the set of all states associated with node $\bli$.  For a state $s$, the DP formulation gives a recursive definition of the values $\soli[s]$ and $\vali[s]$.  $\soli[s]$ is a subset $S$ of $\Xi^+$ that achieves the optimium coverage for $\Gi$ and satisfies additional constraints specified by the state $s$. $\vali[s]$ is the value $\Ci(\Xi^+,\soli[s])$.  
%A state consists of an integer budget, a set of vertices to be in the solution from the bag $X_i$, and for each vertex $u \in X_i$ not in the solution, the number of neighbors in the desired solution from the bags in the sub-tree $\TD_\bli$  and the number of neighbors from the ancestor bags of $\bli$. 
A state $s$ at the node $\bli$ is a tuple $(b, \gamma, \alpha, \beta)$, where
\begin{itemize}
\item $0 \leq b \leq k$ is an integer and specifies the size of $\soli[s]$,
\item $\gamma:\Xi\to \{0,1\}$ is an indicator function for the vertices of $\Xi$. This specifies the constraint that
$\gamma^{-1}(1) \subseteq \soli[s]$ and $\gamma^{-1}(1) \cap \soli[s] = \emptyset$.  We use  $A$ to denote $\cg\inv(1)$ and the state will be clear from the context.
%For each vertex $u \in \Xi$, $\gamma(u)$ indicates whether $u$ is included . % corresponding to the state.
\item $\alpha:\Xi\to [0,k]$ is a function. The constriant is that for each vertex $u \in \gamma\inv(0)$, $u$ should have $\alpha(u)$ neighbors in $\soli[s]$.
\item $\beta: \Xi \to [0,k]$ is function. The constraint is that for each $u \in \gamma\inv(0)$, the weight of $s$ in this state is to be considered as $\wt_s(u) = \wt(u)(1-p)^{\beta(u)}$. 
%{\bf This constraint enables to extend $\soli[s]$ at ancestor nodes of $\bli$ such that $u$ will not be in the solution and should have $\alpha(u) + \beta(u)$ neighbors.}
%in the solution for $\G$ but not in $\Gi$. }%That is, $\beta(u)$ neighbors of $u$ from $V\setminus \Xi^+$ will be added to the solution in the later stage of the dynamic program.
\end{itemize}
{\bf The coverage problem at state $s$}: The PBDS instance at state $s$ is $( \Gi = (\Xi^+, E(\Xi^+), p, \wt_s))$ and budget $b$. $\wt_s$ is defined as follows: For each $u \in \Xi^+$, 
\begin{equation}
\label{eqn:twdpws}
\wt_s(u) = \begin{cases}
\big((1-p)^{\cb(u)}\big)\wt(u) & \text{ if } u \in \Xi \text{ and } c(u) = 0,\\
\wt(u) & \text{ otherwise,}
\end{cases}
\end{equation}
\noindent
In  the following presentation the usage of $\Gi$ and $\mathcal{C}_\bli$ will always be at a specfic state which will be made clear in the context.  
%The functions $\sol_\bli : \S_\bli \to 2^V\cup\{\texttt{undefined}\}$ and $\val_\bli : \S_\bli \to \mathbb{Q}\cup\{\texttt{undefined}\}$ are defined as follows:
%For each state $s = (b,\cg,\ca,\cb)$, t
$\soli[s]$ is a subset of $\Xi^+$ which satisfies all the constraints specified by state $s$ and $\vali[s]=\Ci(\Xi^+,\soli[s]S)$ is the maximum value among $\Ci(\Xi^+,S)$ over all $S \subseteq \Xi^+$ and $|S| \leq b$.
In other words it is the optimum solution for Uni-{\sc PBDS} problem on instance $\langle \Gi, b\rangle$ and it satisfies the constraints specified by $s$.
%\begin{itemize}
%\wt(u) & \text{ if } u \in \Xi \text{ and } c(u) = 1,\\
%\wt(u) & \text{ if } u \notin \Xi.
%\item $\soli[s] \cap \Xi = \cg\inv(1)$,
%\item For each $u \in \Xi$ with $c(u) = 0$, $|N(u) \cap \Xi^+ \cap \soli[s]| = \ca(u)$, and
%\item $\vali[s] = \Ci(\Xi^+, \soli[s])$, where the coverage function $\Ci(\cdot)$ denotes $\C_{\Gi}()$ where the vertex weights of $\Gi$ are governed by $\wt_s$. We use this notation of coverage function thought out this section and in Appendix~\ref{apdx:sec:dp}. 
%\end{itemize}
%where the weight function $\wt^s:\Xi^+ \to \mathbb{R}$ is defined as follows: For each vertex $u \in \Xi^+$,
%\[\wt^s_u = \begin{cases}
%\big((1-p)^{\cb(u)}\big)\wt_u & \text{ if } u \in \Xi \text{ and } c(u) = 0,\\
%\wt_u & \text{ if } u \in \Xi \text{ and } c(u) = 1,\\
%\wt_u & \text{ if } u \notin \Xi.
%\end{cases}\]
A state $s = (b,\cg,\ca,\cb)$ at a node $\bli$ is said to be \emph{invalid} if there no feasible solution that satisfies the constraints specified by $s$, and $\soli[s] = \texttt{undefined}$ and $\vali[s] = \texttt{undefined}$. If there is a feasible solution, the state is called valid. \\  

  \noindent
{\bf State induced at a node in $\TD$ by a set}:
% and we mark the solutions of the invalid states as \texttt{undefined}.
For a set $D \subseteq V$ of size $k$, we say that $D$ {\em induces} a state $s=(b,\cg, \ca, \cb)$ at node $\bli$
and $s$ is defined as follows:
\begin{itemize}
\item $b = |D \cap \Xi^+|$,
\item The function $\cg:\Xi\to\{0,1\}$ is defined as follows- for each $u\in D \cap \Xi$, $\cg(u) = 1$ and $\cg(u)=0$, for each $u \in D \setminus \Xi$.
\item The functions $\ca, \cb:\Xi\to[0,k]$ are defined as follows-  for each $u\in \cg\inv(0)$, $\ca(u) = |N(u) \cap \Xi^+ \cap D|$, and $\cb(u) = |N(u) \cap (V\setminus \Xi^+) \cap D|$.
%\item $\cb:\Xi\to[0,k]$ such that for each $u\in \Xi$, $\cb(u) = |N(u) \cap (V\setminus \Xi^+) \cap D|$.
\end{itemize}
Depending on $\ca$ and $\cb$ that there can be  different states induced by a set $D$.
%\begin{comment}
\subsection{Recursive definition of $\soli$ and $\vali$}
\label{sec:recdef}
For each node $\bli \in V(\TD)$  and $s = (b,\cg,\ca,\cb) \in \Si$, we show how to compute $\soli[s]$ and $\vali[s]$ from the  tables at the children of $\bli$.  $\soli[s]$ and $\vali[s]$ are recursively defined below and we prove a statement on the structure of an optimal solution based on the type of the node $\bli$ in $\TD$.
These statements are used in Section \ref{sec:bottomup} to prove the correctness of the bottom-up evalution.  
%\noindent
% {\em Notation:} We use  $A$ to denote $\cg\inv(1)$. Recall that at state $s$, $w_s(u) = (1-p)^{\cb(u)}w(u)$. \\
%

\noindent {\bf Leaf node}: Let $\bli$ be a leaf node with bag $\Xi = \emptyset$. The state set $\S_\bli$ is a singleton set with a state $s = (0, \emptyset\to\{0,1\}, \emptyset\to[k], \emptyset \to [k])$. Therefore,
$\soli[s] = \emptyset \text{ and } \vali[s] = 0.$
This can be computed in constant time.
\begin{lemma}
\label{lem:leaf}
The table entries for the state $s$ at a leaf node is computed optimally. 
\end{lemma}
\begin{proof}
The correctness follows from the fact that the graph $\Gi$ is a \emph{null graph}. 
Thus, for a null graph and a valid state $s$, empty set with coverage value zero is the only optimal solution. 
\end{proof}
\noindent {\bf Introduce node}: Let $\bli$ be an introduce node with child $\blj$ such that $\Xi = \Xj \cup \{v\}$ for some $v \notin \Xj$.  
Since $\bli$ is an introduce node, all the neighbors of $v$ in $\G[\Xi^+]$ are in $\Xi$. 
Thus, $N(v) \cap \Xi^+ = N(v) \cap \Xi$.   
In case, $\alpha(v) \not= |N(v) \cap A|$, then, by definition of a solution at a state, the state $s$ does not have a feasible solution. 
Therefore, the state $s$ is invalid. 
Next consider that in state $s$,  $\alpha(v) = |N(v) \cap A|$,
We  define the state $s_\blj$ and define $\soli[s]$ in terms of $\solj[s_\blj]$. 
The state $s_\blj$ differs based on whether $\cg(v) = 0$ and $\cg(v) = 1$. 
For the case  $\cg(v)=0$ the solution to be computed for the state $s$ must not contain $v$, and  for the case $\cg(v)=1$, solution to be computed must contain $v$.  

\noindent
In the case $\cg(v)=0$, define $s_\blj = (b, \cg_\blj, \ca_\blj, \cb_\blj)$ to be the state from  node $\blj$ where
the functions $\cg_\blj:\Xj\to\{0,1\}$, $\alpha_\blj:\Xj\to[0,k]$ and $\beta_\blj:\Xj\to[0,k]$ are as follows:  for each $u \in \Xj$, $\cg_\blj(u) = \cg(u)$, $\alpha_\blj(u) = \alpha(u)$ and $\beta_\blj(u) = \beta(u)$. 
If the state $s_\blj$ is invalid then the state $s$ is also invalid. 
Therefore, we consider that the state $s_\blj$ is valid. 
Then the solution at state $s$ as follows:
%$\soli[s]$ and $\vali[s]$ are defined as follows:\\
\begin{equation}
\label{eqn:dpinsolcv0}
\soli[s] = \solj[s_\blj] 
\end{equation}
and
\begin{equation}
\label{eqn:dpinvalcv0}
\vali[s] = \valj[s_\blj]+\big( 1- (1-p)^{\ca(v)} \big)\wt_s(v)
\end{equation}
\noindent Next, we consider the second case that $\cg(v) = 1$. 
Let $D_v = N(v) \cap \cg\inv(0)$, that is the set of neighbors of $v$ which are not to be selected in $\soli[s]$.
Indeed, these vertices must be considered as their contribution to the expected coverage will increased due to the {\em introduction} of $v$.  
Let $s_\blj = (b-1, \cg_\blj, \ca_\blj, \cb_\blj)$ be the state in the node $\blj$ where
the functions $\cg_\blj:\Xj\to\{0,1\}$, $\alpha_\blj:\Xj\to[0,k]$ and $\beta_\blj:\Xj\to[0,k]$ are defined as follows:  for each $u \in \Xj$, $\cg_\blj(u) = \cg(u)$,
$$\alpha_\blj(u) = \begin{cases} \alpha(u)-1 & \text{ if } u \in D_v,\\
\alpha(u) & \text{ otherwise},\end{cases}$$ 
and $$\beta_\blj(u) = \begin{cases} \beta(u)+1 & \text{ if } u \in D_v,\\
\beta(u) & \text{ otherwise}.\end{cases}$$  
Note the increase and decrease of $\alpha$ and $\beta$ at each $u \in D_v$: this is to take care of the fact that
a neighbor $v$ has been introduced at node $\bli$ and the aim is to compute a solution that contains $v$. Therefore, at $s_\blj$ for each $u \in \cg\inv(0)$ we consider $\alpha_\blj(u) = \alpha(u)-1$ to reflect the fact that $v$ is not in $\Xj$. To ensure that the solution computed at state $s_\blj$ gives us the desired solution at $s$, for each $u \in \cg\inv(0)$ we consider $\beta_\blj(u) = \beta(u)+1$. Recall that this ensures that $\wt_{s_\blj}(u) = (1-p)^{\beta(u)+1}\wt(u) = (1-p)\wt_s(u)$.  This is used in the coverage expressions in the proof of Lemma \ref{lem:intr}.

\noindent
We now define $\soli[s]$ and $\vali[s]$.
If the state $s_\blj$ is invalid then the state $s$ also invalid. 
Therefore, we consider that the state $s_\blj$ is valid. 
The solution for the state $s$ is defined as follows:
\begin{equation}
\label{eqn:dpinsolcv1}
\soli[s] = \solj[s_\blj] \cup \{v\}
\end{equation}
and 
\begin{equation}
\label{eqn:dpinvalcv1}
\vali[s] = \valj[s_\blj] + \sum_{u \in D_v} p(1-p)^{\alpha(u)-1}\wt_s(u) + \wt_s(v)
\end{equation}
In both the cases, the state $s_\blj$ can be computed in $\Oh(w)$ time. 

\begin{lemma}
\label{lem:intr}
Let $\bli$ be an introduce node in $\TD$ and let $s$ and $s_\blj$ be as defined above.  Let $S$ be a solution of optimum coverage at the state  $s$, then $S \setminus \{v\}$ gives the optimum coverage at the state $s_\blj$ in the node $\blj$.
\end{lemma}
\begin{proof}
Since $S$ is solution at state $s$, by definition $S$ induces the state $s$ at node $\bli$.  
In this proof $\Ci(\Xi^+,S)$ is the coverage at state $s$ and $\Cj(\Xj^+,S)$ is the coverage at state $s_\blj$.
The proof technique is to rewrite $\Ci(\Xi^+,S)$ as a sum of $\Cj(\Xj^+,S \setminus \{v\})$ and an additional term that depends only on $v$, its neighborhood and the state $s$.  This shows that $S \setminus \{v\}$ induces the state $s_\blj$ and attains the maximum coverage at $s_\blj$. 
We consider two cases based on whether $v \in A$ or not. 
In the case $v\notin A$, first it follows that $v \notin S$. Further, by definition 
we have $\Ci(\Xi^+, S) = \Ci(\Xi^+\setminus\{v\}, S) + \Ci(v,S)$. 
Since $s_\blj$ is identical to $s$ except for the vertex $v$ which is not in $\Xj$, it follows that for each $u \in \Xj$, $\wt_{s_{\blj}}(u) = \wt_s(u) $. Therefore,  $\Cj(\Xj^+, S) = \Ci(\Xi^+\setminus\{v\}, S) $.  Further, the state induced by the solution $S$ at node $\blj$ is the state $s_\blj$, and in this case
$S \setminus \{v\}$ is $S$ itself. Therefore, the optimum coverage at $s_\blj$ is achieved by $S \setminus \{v\}$. 

\noindent In the case $v\in A$, it follows that $v \in S$. Further, by definition of $s_\blj$, and the fact that $S$ induces the state $s$, it follows that  $S\setminus \{v\}$ induces the state $s_\blj$.
The coverage value $\Ci(\Xi^+, S)$ can be written as follows:
\begin{eqnarray*}
\Ci(\Xi^+, S) &=& \Ci(\Xi^+\setminus \Xi, S) + \Ci(\Xi\setminus(D_v \cup \{v\}), S) + \Ci(D_v, S) + \Ci(v,S)\\
&=& \Cj(\Xj^+\setminus \Xj, S\setminus\{v\}) + \Cj(\Xj\setminus D_v, S\setminus\{v\}) + \Ci(D_v, S) + \wt_s(v)
\end{eqnarray*}
The first equality follows by partitioning $\Xi^+$ into four sets so that the coverage of each set by $S$ summed up gives the coverage of $\Xi^+$ by $S$. 
In the second equality, the first two terms are re-written as coverage by $S \setminus \{v\}$ at node $\blj$, and $\Ci(v,S)$ is re-written as $\wt_s(v)$.  Since $\bli$ is an introduce node,  the key facts used in this equality are that $\Xi^+\setminus \Xi = \Xj^+\setminus \Xj$ and $\Xi \setminus(D_v \cup \{v\} =  \Xj\setminus D_v$. The other key facts used are that
$\cg_\blj$ and $\gamma$ are identical on $\Xj$, $\ca_\blj$ and $\ca$ are identical on $\Xj^+\setminus \D_v$, and $\cb_\blj$ and $\cb$ are identical on $\Xj^+\setminus \D_v$.  
The coverage value of $\Ci(D_v, S)$ is now re-written as follows, using the key fact that for all $u \in \D_v$, $\gamma(u) = 0$, and $|N(u) \cap S| = \alpha(u)$, and that the state induced by solution $S$ at node $\bli$  is the state $s$:
\begin{eqnarray*}
\Ci(D_v, S) &=& \sum_{u \in D_v} \Ci(u,S) = \sum_{u \in D_v} (1-(1-p)^{|N(u) \cap S|})\wt_s(u) = \sum_{u \in D_v} (1-(1-p)^{\ca(u)})\wt_s(u)\\
&=& \sum_{u \in D_v} (1-(1-p)^{\ca(u)})(1-p)^{\cb(u)}\wt(u)\\ 
&=& \sum_{u \in D_v} \Big(\big(1-(1-p)^{\ca(u)-1}\big)(1-p)^{\cb(u)+1} + p(1-p)^{\ca(u)-1}(1-p)^{\cb(u)}\Big)\wt(u)\\
&=& \sum_{u \in D_v} \Big(\big(1-(1-p)^{\ca(u)-1}\big)\wt_{s_\blj}(u) +  \sum_{u \in D_v}p(1-p)^{\ca(u)-1}\wt_s(u)\\
&=& \sum_{u \in D_v} \Cj(u, S\setminus\{v\}) +  \sum_{u \in D_v}p(1-p)^{\ca(u)-1}\wt_s(u)\\
&=& \Cj(D_v, S\setminus\{v\}) + \sum_{u \in D_v}p(1-p)^{\ca(u)-1}\wt_s(u)
\end{eqnarray*}
By substituting the value of $\Ci(D_v, S)$ into $\Ci(\Xi^+,S)$, we  get the following:
\begin{eqnarray*}
\Ci(\Xi^+, S) &=& \Cj(\Xj^+\setminus D_v, S\setminus\{v\}) + \Cj(D_v, S\setminus\{v\}) + \sum_{u \in D_v}p(1-p)^{\ca(u)-1}\wt_s(u) + \wt_s(v)\\
&=& \Cj(\Xj^+, S\setminus\{v\}) + \sum_{u \in D_v}p(1-p)^{\ca(u)-1}\wt_s(u) + \wt_s(v)
\end{eqnarray*}
In this case also, we have rewritten $\Ci(\Xi^+, S)$ as sum of  $\Cj(\Xj^+, S\setminus\{v\})$  and term dependent on $v$ and the state $s$.  
Thus, since $S$ is an optimal solution for state $s$ in $\bli$, it follows that $S \setminus \{v\}$ is an optimal solution for the state $s_\blj$ in $\blj$. %Hence the lemma.
\end{proof}

\noindent {\bf Forget node}: Let $\bli$ be a forget node with child $\blj$ such that $\Xi = \Xj \setminus \{v\}$ for some $v \in \Xj$.
Since $\bli$ is a forget node,  $N(v) \cap (V\setminus \Xi^+) = \emptyset$, that is, 
all neighbors of $v$ in $\G$ are in $\Gi$. Further, for each vertex $u \in \Xi$, $N[u] \cap \Xi^+ = N[u] \cap \Xj^+$. 
We define the state $s_\blj$ and define $\soli[s]$ in terms of $\solj[s_\blj]$. 
We  consider all possible values of $\cg(v)$, $\ca(v)$, and $\cb(v)$ to define the state $s_\blj$. 
These values specify the different states in $\blj$. 
For each $z \in \{0,1\}$, define $\cg^z:\Xj \to \{0,1\}$ as follows: for each $u \in \Xj$, $$\cg^z(u) = \begin{cases} \cg(u) & \text{ if } u \not= v,\\
z & \text{ u = v }.\end{cases}$$ 
The parameter $z$ specifies  whether $v$ should be in the desired solution or not. 
For each $x \leq [0,b]$, define $\alpha^{x}:\Xj \to [0,k]$ as follows: $$\alpha^{x}(u) = \begin{cases} \alpha(u) & \text{ if } u \not= v,\\
x & \text{ u = v.}\end{cases}$$ 
In the case when $\cg^{z}(v)=0$,  then the parameter $x$ specifies the number of neighbors of $v$ which should be in the desired solution. 
Define $\beta':\Xj \to [0,k]$ as follows: $$\beta'(u) = \begin{cases} \beta(u) & \text{ if } u \not= v,\\
0 & \text{ u = v.}\end{cases}$$ 
For each $z \in \{0,1\}$ and each $x \in [0,b]$, let $s^{z,x}$ denote the state $(b, \cg^z, \alpha^{x}, \beta')$ in $\blj$. \\
If for each $z \in \{0,1\}$ and each $x \in [0,b]$,  $s^{z,x}$ is invalid, then the state $s$ also invalid. 
Therefore, we consider that there exists a 2-tuple $z \in \{0,1\}$ and each $x \in [0,b]$ such that the state $s^{z,x}$ is valid. 
Further, we define the following 2-tuple as follows:
\begin{equation}
\label{eqn:dpfnargmax}
z',x' = \argmax_{\substack{z \in \{0,1\}, x \in [0,b]\\ s^{z,x}\text{ is valid}}} \valj[s^{z,x}].
\end{equation} 
Define $s_\blj = s^{z',x'} = (b, \cg^{z'},\alpha^{x'}, \beta')$ and the solution at the state $s$ as follows:
\begin{equation}
\label{eqn:dpfnsol}
\soli[s] = \solj[s_\blj],
\end{equation}
and
\begin{equation}
\label{eqn:dpfnval}
\vali[s] = \valj[s_\blj].
\end{equation}
The state $s_\blj$ can be computed in $\Oh( k)$ time.
\begin{lemma}
\label{lem:forget}
Let $\bli$ be a forget node in $\TD$, and let $s$ and $s_\blj$ be as defined above. If $S$ is a solution of optimum coverage at state $s$, then $S$ is a solution of optimum coverage at the state $s_\blj$ in node $\blj$. 
\end{lemma}
\begin{proof}
Let $\hat{s}$ be the state induced by $S$ in the node $\blj$. In the following argument, the coverage $\Ci(\Xi^+,S)$ is considered at state $s$ and the coverage $\Cj(\Xj^+,S)$ is considered at state $\hat{s}$ in node $\blj$.
Since $\Xi^+ = \Xj^+$, $\Ci(\Xi^+, S) = \Ci(\Xj^+, S) = \Cj(\Xj^+, S) = \valj[\hat{s}]$. 
Let us define $z = |\{v\} \cap S|$ and $x = |N[z] \cap S|$.  From Equation~\ref{eqn:dpfnargmax}, it is clear that the $z', x'$ chosen is such that $\valj[s^{z',x'}] \geq \valj[s^{z,x}] = \valj[\hat{s}]$. Since $s_\blj$ is defined as $s^{z',x'}$, $\valj[s_\blj] \geq \valj[s^{z,x}] = \valj[\hat{s}] = \Cj(\Xj^+,S)$.  Since $S$ is an optimal solution at state $s$, and since $\Xi^+ = \Xj^+$, it follows that $\Cj(\Xj^+,S) \geq \valj[s_\blj]$.  Therefore $\vali[s] = \Ci(\Xi^+,S) = \Cj(\Xj^+,S) = \valj[s_\blj]$. Hence the lemma.
%Thus, since $S$ is an optimal solution for state $s$ in node  $\bli$, it follows that $S$ is an optimal solution for the state $s_\blj$ in $\blj$. 
\end{proof}

\noindent {\bf Join node}: Let $\bli$ be a join node with children $\blj$ and $\blh$ such that $\Xi = \Xj = \Xh$. 
We define the states $s_\blj$ and $s_\blh$, and define $\soli[s]$ in terms of $\solj[s_\blj]$ and $\solh[s_\blh]$.  $s_\blj$ and $s_\blh$ are selected from a set consisting of $O(k^\omega)$ elements.  

\noindent
To define $s_\blj$ and $s_\blh$, we observe that since $\Xi = \Xj = \Xh$, $\cg\inv(1)$ is contained in both $\Xj$ and $\Xh$. Therefore, the $\cg$ gets carried over  from $s$ to $s_\blj$ and $s_\blh$.

\noindent
Next, we identify the candidate values for the budget in the two states $s_\blj$ and $s_\blh$.  We know that in a solution $S$ which induces the state $s$ at node $\bli$ , $|\cg\inv(1)|$ vertices are in $\Xi$ and $b-|\cg\inv(1)|$ vertices are in $\Xi^+\setminus \Xi$. 
Since $\Xi^+\setminus \Xi$ can be partitioned into two sets $\Xj^+\setminus \Xj$ and $\Xh^+\setminus \Xh$, we consider a parameter $z$ to  partition the value $b-|\cg\inv(1)|$. 
For each $0 \leq z \leq b-|\cg\inv(1)|$, let $b_{\blj,z} = |\cg\inv(1)| + z$ and $b_{\blh,z} = b-z$: we consider states at nodes $\blj$ and $\blh$ with { budget} $b_{\blj,z}$ and $b_{\blh,z}$, respectively.  In other words, for each $0 \leq z \leq b-|\cg\inv(1)|$, we search for a solution of size $b_{\blj,z}$ for a subproblem on $\Xj^+$ which contains $\cg\inv(1)$ and $z$ vertices from $\Xj^+ \setminus \Xj$.  Symmetrically, in node $\blh$, we search for a solution of size $b_{\blh,z}$ for a subproblem on  $\Xh^+$ which contains $\cg\inv(1)$ and $b-\cg\inv(1)-z$ vertices from $\Xh^+ \setminus \Xh$.  These two solutions taken together gives a solution fo size $b$ at state $s$ in node $\bli$.  To ensure that the constraints specified by $\ca$ and $\cb$ are met, we next consider appropriate candidate functions in $s_\blj$ and $s_\blh$.\\

\noindent
 The different candidate functions to obtain $\ca_\blj$ and $\ca_\blh$ in the states $s_\blj$ and $s_\blh$, respectively are based on the coverage of vertices in $\cg\inv(0)$. For each $u \in \cg\inv(0)$, $\alpha(u)$ and $\beta(u)$ are  distributed between $s_\blj$ and $s_\blh$, respectively. The number of possible ways in which this can be done is defined by the following set $\A$.  
Let $$ \A = \{\eta:\cg\inv(0) \to [0,b] \mid \text{for each } u \in \cg\inv(0), 0 \leq \eta(u) \leq \alpha(u)-|N(u) \cap \cg\inv(1)|\}. $$ 
A function $\eta \in \A$ specifies that for each $u \in \cg\inv(0)$, $|N(u) \cap \cg\inv(1)|+\eta(u) $  neighbors of $u$  from $\Xj^+$ should be in the solution from the node $\blj$ and $\alpha(u)-\eta(u)$  neighbors of $u$ from $\Xh^+$ should be in the solution from the node $\blh$.  In particular, in the solution at node $\blj$, $\eta(u)$ neighbours of $u$ must be in $\Xj^+ \setminus \Xj$ and, in the solution at node $\blh$, $\alpha(u) - \eta(u) - |N(u) \cap \cg\inv(1)|$ neighbors of $u$ must be in $\Xh^+ \setminus \Xh$.
More precisely, for each $\eta \in \A$, we define the following functions. 
Let $\alpha_{\blj,\eta}:\Xj\to[0,k]$ such that for each $u \in \Xj$,
$$ \alpha_{\blj, \eta}(u) = \begin{cases} \alpha(u) & \text{ if } \cg(u) = 1,\\
|N(u) \cap \cg\inv(1)| + \eta(u) & \text{ if } \cg(u) = 0.\end{cases}$$
Let $\alpha_{\blh,\eta}:\Xh\to[0,k]$ such that for each $u \in \Xh$,
$$ \alpha_{\blh, \eta}(u) = \begin{cases} \alpha(u) & \text{ if } \cg(u) = 1,\\
\alpha(u)-\eta(u) & \text{ if } \cg(u) = 0.\end{cases}$$
Note that $N(u) \cap \cg\inv(1)$ is counted in both the nodes $\blj$ and $\blh$, and we take care of this after  identifying the candidates functions for $\beta_\blj$ and $\beta_\blh$. Recall, that at state $s$ in node $\bli$, for each $u \in \cg\inv(0)$,  $\soli[s]$ provides a coverage value for $u$ as if it has $\alpha(u) + \beta(u)$ neighbors in $\soli[s]$.  Among these, exactly $\alpha(u)$ must be selected from $\Xi^+$.  To ensure that this constraint is met, we consider the following candidate functions for $\beta_{\blj}$ and $\beta_{\blh}$.\\
For each $\eta \in \A$, define $\beta_{\blj,\eta}:\Xj\to[0,k]$ such that for each $u \in \Xj$,
$$ \beta_{\blj, \eta}(u) = \begin{cases} \beta(u) & \text{ if } \cg(u) = 1,\\
\beta(u) + \alpha(u)-|N(u) \cap \cg\inv(1)|-\eta(u) & \text{ if } \cg(u) = 0.\end{cases}$$
Observe that $\alpha_{\blj,\eta}(u)=|N(u) \cap \cg\inv(1)|-\eta(u)$ is subtracted from $\alpha(u)+\beta(u)$. Symmetrically, $\alpha_{\blh,\eta}(u)$ is  subtracted from $\alpha(u)+\beta(u)$ to obtained a candidate $\beta_\blh$.
Let $\beta_{\blh,\eta}:\Xh\to[0,k]$ such that for each $u \in \Xh$,
$$ \beta_{\blh, \eta}(u) = \begin{cases} \beta(u) & \text{ if } \cg(u) = 1,\\
\beta(u) + \eta(u) & \text{ if } \cg(u) = 0.\end{cases}$$ \\

\noindent
Using the candidate values for budget, $\cg$, $\ca$, and $\cb$ at  node $\blj$ and node $\blh$, we now specify the set of candidate states to be considered at nodes $\blj$ and $\blh$.
For each $0 \leq z \leq b-|\cg\inv(1)|$ and each $\eta \in \A$, let $s_{\blj,z,\eta} = (b_{\blj,z}, \cg, \alpha_{\blj,\eta}, \beta_{\blj,\eta})$ and $s_{\blh,z,\eta} = (b_{\blh,z}, \cg, \alpha_{\blh,\eta}, \beta_{\blh,\eta})$. \\

\noindent
Next, to write $\soli[s]$ in terms of coverage of $\Xj^+$ and $\Xh^+$ we need to identify vertices whose contribution the coverage would be over-counted when we take the union of $\soli[s_\blj]$ and $\soli[s_\blh]$. Since $\Xi = \Xj = \Xh$, two cases need to be handled.
First, the vertices on $\cg\inv(1)$ are counted twice, once in $\Xj$ and once in $\Xh$.  Therefore, in the expansion of $\Ci(\Xi^+, S)$ in terms of the coverage at $\Xj$ and $\Xh$, we will have to subtract out $\sum_{u \in \cg\inv(1)}\wt_s(u)$.  Secondly,  for each $\eta \in \A$ and each $u \in \cg\inv(0)$, the coverage of $u$ by $\cg\inv(1)$ is counted twice, once in $\Xj$ and once in $\Xh$.  To subtract this over-counting we introduce the following function $\lambda$ associated with the state $s$ at the join node $\bli$. It is an easy arithmetic exercise to verify that $\lambda(\eta,u)$ is the value that must be subtracted.
For each $\eta \in \A$ and for each $u \in \cg\inv(0)$, let $$ \lambda(\eta,u) = \big( (1-p)^{\alpha(u)-|N(u) \cap \cg\inv(0)|-\eta(u)} + (1-p)^{\eta(u)} - (1-p)^{\alpha(u)}-1\big)\wt_s(u).$$

\noindent
Finally, we come to the recursive specification of $\soli[s]$. 
If for each $0 \leq z \leq b-|\cg\inv(1)|$ and each $\eta \in \A$, either $s_{\blj,z,\eta}$ or $s_{\blh,z,\eta}$ is invalid, then $s$ is also invalid. 
Therefore, we consider those values of $0 \leq z \leq b-|\cg\inv(1)|$ and $\eta \in \A$ such that both the states $s_{\blj,z,\eta}$ and $s_{\blh,z,\eta}$ are valid. 
Further, we define the following tuple :
\begin{equation}
\label{eqn:dpjnargmax}
z',\eta' = \argmax_{\substack{0 \leq z \leq b-|\cg\inv(1)|, \eta \in \A,\\ s_{\blj,z,\eta} \text{ and } s_{\blh,z,\eta} \text{ are valid}}}\valj[s_{\blj,z,\eta}] + \valh[s_{\blh,z,\eta}] - \sum_{u \in \cg\inv(0)}\lambda(\eta,u)
\end{equation}
Define $s_\blj = s_{\blj,z',\eta'} = (b_{\blj,z'},\cg,\alpha_{\blj,\eta'}, \beta_{\blj,\eta'})$ and $s_\blh = s_{\blh,z',\eta'} = (b_{\blh,z'},\cg,\alpha_{\blh,\eta'}, \beta_{\blh,\eta'})$.
Then, the solution for the state $s$ is defined as follows:
\begin{equation}
\label{eqn:dpjnsol}
\soli[s] = \solj[s_\blj] \cup \solh[s_\blh],
\end{equation}
and
\begin{equation}
\label{eqn:dpjnval}
\vali[s] = \valj[s_\blj] + \valh[s_\blh] - \sum_{u \in \cg\inv(0)} \lambda(\eta',u)-\sum_{u \in \cg\inv(1)}\wt_s(u).
\end{equation}
The cardinality of the set $\mathcal{A}$ is at most $\Oh(k^{w})$. This is the most dominant term in the size of the recursive definition. This is becuase for each fixed $\eta \in \mathcal{A}$, $\ca$ and $\cb$ are uniquely defined.  Then, the states $s_\blj$ and $s_\blh$ can be computed in $\Oh(k^{w+1}wn)$ time. 
%{\bf Need to discuss the statement of join node}
\begin{lemma}
\label{lem:join}
Let $s$ be a state in the join node $\bli$ in $\TD$ and let $s_\blj$ and $s_\blh$ be as defined above. 
Let $S$ be a solution of optimum coverage at state $s$, then $\Ci(\Xi^+, S) \leq \vali[s]$.
%$S$ is a solution of optimum coverage at 
%states $s_\blj$ and $s_\blh$ at nodes $\blj$ and $\blh$, respectively.
%Let $S_{\blj} = S \cap \Xj^+$ and $S_{\blh} = S \cap \Xh^+$, then $S_\blj$ and $S_\blh$ give optimum coverage for the states $s_\blj$ and $s_\blh$, respectively. 
\end{lemma}
\begin{proof}
Let $\hat{s} = (\hat{b}, \hat{\cg}, \hat{\ca}, \hat{\cb})$ and $\tilde{s} =(\tilde{b}, \tilde{\cg}, \tilde{\ca}, \tilde{\cb})$ be the  states induced at the nodes $\blj$ and $\blh$ by the set $S$, respectively.
In this context, we consider the coverage functions $\Ci(\cdot,\cdot)$, $\Cj(\cdot,\cdot)$ and $\Ch(\cdot,\cdot)$ are considered at states $s$, $\hat{s}$ and $\tilde{s}$, respectively. \\
%$S_\blj$ and $S_\blh$, respectively. 
Let $S_\blj = S \cap (\Xj^+ \setminus \Xj)$ and $S_\blh = S \cap (\Xh^+ \setminus \Xh)$.
Let $z = |S_\blj|$ and $\eta:\cg\inv(0)\to[0,b]$ such that for each $u \in \cg\inv(0)$, $\eta(u) = N(u) \cap (\Xj^+\setminus \Xj)$.   We now define $\Ci(\Xi^+, S)$ in terms of $\Cj(\Xj^+, S)$, $\Ch(\Xh^+, S)$, and a subtracted term dependent on $z$, $\eta$, and $s$.  This is done as follows and we ensure that the coverage is exactly counted. 
\begin{eqnarray}
\Ci(\Xi^+, S) &=& \Ci(\Xi^+\setminus\Xi, S) + \Ci(\Xi, S) \nonumber\\
&=& \Ci(\Xj^+\setminus \Xj, S) + \Ci(\Xh^+\setminus \Xh, S) + \Ci(\cg\inv(1), S) + \Ci(\cg\inv(0), S) \nonumber \\
&=& \Cj(\Xj^+\setminus \Xj, S_\blj) + \Ch(\Xh^+\setminus \Xh, S_\blh) + \Ci(\cg\inv(1), S) + \sum_{u \in \cg\inv(0)} \Ci(u, S) \label{eqn:cov-expan}
\end{eqnarray}
The first equality follows by the partition $\Xi^+$ into $\Xi^+\setminus \Xi$ and $\Xi$. 
In the second equality, the set $\Xi^+\setminus \Xi$ is partitioned into $\Xj^+\setminus \Xj$ and $\Xh^+ \setminus \Xh$, and the set $\Xi$ is partitioned in $\cg\inv(0)$ and $\cg\inv(1)$.
The third equality  follows from the fact that for each $u \in \Xj^+\setminus \Xj$, $\wt_{\hat{s}}(u) = \wt_s(u)$ and $N[u] \cap S = N[u] \cap S_\blj$. 
Similarly, for each $u \in \Xh^+\setminus \Xh$, $ \wt_{\hat{s}}(u)= \wt_s(u)$ and $N[u] \cap S = N[u] \cap S_\blh$. \\

\noindent
Next, we consider the term $\sum_{u \in \cg\inv(0)} \Ci(u, S) $.  For each $u \in \cg\inv(0)$, $\Ci(u,S)$ can be written as sum of coverages of $u$ by the sets $S_\blj$ and $S_\blh$. In particular, here we carefully use the values of $\hat{\ca}$ and $\hat{\cb}$ at node $\blj$ and $\tilde{\ca}$ and $\tilde{\cb}$ at node $\blh$. Further, each of the equations follows by simple arithmetic and the definition of $\Cj(u,S_\blj)$, $\Cj(u,S_\blh)$, $\hat{\alpha}$, and $\tilde{\alpha}$.
\begin{eqnarray*}
\Ci(u, S) &=& \big(1-(1-p)^{\alpha(u)}\big)\wt_s(u) \\
&=& \big(1-(1-p)^{\ca(u)}\big)(1-p)^{\cb(u)}\wt(u)\\
&=& \Big(\big(1-(1-p)^{\hat{\ca}(u)}\big)(1-p)^{\hat{\cb}(u)}\wt(u)\Big) + \Big(\big(1-(1-p)^{\tilde{\ca}(u)}\big)(1-p)^{\tilde{\cb}(u)}\wt(u)\Big)\\
&& - \big( (1-p)^{\hat{\ca}(u)-\cg\inv(1)} + (1-p)^{\tilde{\ca}(u)-\cg\inv(1)} - (1-p)^{\ca(u)}-1\big)(1-p)^{\cb(u)}\wt(u)\\
&=& \Cj(u, S_\blj) + \Ch(u, S_\blh)\\
&& - \big( (1-p)^{|N(u) \cap (\Xj^+\setminus \Xj)|} + (1-p)^{|N(u) \cap (\Xh^+\setminus \Xh)|} - (1-p)^{\alpha(u)}-1\big)\wt_s(u)\\
&=& \Cj(u, S_\blj) + \Ch(u, S_\blh)\\
&& - \big( (1-p)^{\alpha(u)-|N(u) \cap \cg\inv(0)|-\eta(u)} + (1-p)^{\eta(u)} - (1-p)^{\alpha(u)}-1\big)\wt_s(u)\\
&=& \Cj(u, S_\blj) + \Ch(u, S_\blh) - \lambda(\eta, u)
\end{eqnarray*}
We substitute this in Equation \ref{eqn:cov-expan} and derive the following equalities.
\begin{eqnarray*}
\Ci(\Xi^+, S)&=& \Cj(\Xj^+\setminus \Xj, S_\blj) + \Ch(\Xh^+ \setminus \Xh, S_\blh) + \Ci(\cg\inv(1), S)\\  
&& + \sum_{u \in \cg\inv(0)} \Big(\Cj(u, S_\blj) + \Ch(u, S_\blh) - \lambda(\eta, u)\Big)\\
&=& \Cj(\Xj^+ \setminus \Xj, S_\blj) + \Ch(\Xh^+ \setminus \Xh, S_\blh) + \Cj(\cg\inv(0), S_\blj) + \Ci(\cg\inv(1), S) \\
&& + \Ch(\cg\inv(0), S_\blh) + \Ci(\cg\inv(1), S)  - \Ci(\cg\inv(1), S) -\sum_{u \in \cg\inv(0)}\lambda(\eta, u)
\end{eqnarray*}
Using $\hat{\alpha}$ and $\hat{\beta}$, it follows that  $\Cj(\Xj, S) = \Cj(\cg\inv(0), S_\blj) + \Ci(\cg\inv(1), S)$. Similarly, using $\tilde{\alpha}$ and $\tilde{\beta}$, it follows that  $\Ch(\Xh, S) = \Ch(\cg\inv(0), S_\blh) + \Ci(\cg\inv(1), S)$. Therefore,
\begin{eqnarray*}
\Ci(\Xi^+, S)&=& \Cj(\Xj^+ \setminus \Xj, S_\blj) + \Ch(\Xh^+ \setminus \Xh, S_\blh) + \Cj(\Xj, S) + \Ch(\Xh, S) \\
&&  - \Ci(\cg\inv(1), S) -\sum_{u \in \cg\inv(0)}\lambda(\eta, u) 
\end{eqnarray*}
Putting together the terms corresponding to $\Cj(\cdot,\cdot)$ and $\Ch(\cdot,\cdot)$ it follows that
\begin{eqnarray*}
\Ci(\Xi^+, S)&=& \Cj(\Xj^+, S) + \Ch(\Xh^+, S) -  \Ci(\cg\inv(1), S) -\sum_{u \in \cg\inv(0)}\lambda(\eta, u) 
\end{eqnarray*}
Since $\hat{s}$ and $\tilde{s}$ are states at nodes $\blj$ and $\blh$ induced by the state $S$, we know that
$\Cj(\Xj^+, S) \leq  \valj[\hat{s}]$ and $\Ch(\Xh^+, S) \leq \valh[\tilde{s}]$.  Therefore, 
\begin{eqnarray*}
\Ci(\Xi^+, S) &\leq& \valj[\hat{s}] + \valh[\tilde{s}]  - \sum_{u \in \cg\inv(1)}\wt_s(u) - \sum_{u \in \cg\inv(0)} \lambda(\eta, u)
\end{eqnarray*}
Further, by the choice of $z',\eta'$ in Equation ~\ref{eqn:dpjnargmax}, we know that $\hat{s}$ and $\tilde{s}$ do not result in a larger value than $s_{\blj}$ and $s_{\blh}$.  Formally,   we know that
\begin{eqnarray*}
\valj[\hat{s}] + \valh[\tilde{s}]  - \sum_{u \in \cg\inv(1)}\wt_s(u) - \sum_{u \in \cg\inv(0)} \lambda(\eta, u) \leq \vali[s]
\end{eqnarray*}
Hence the Lemma.
%By Equation~\ref{eqn:dpjnargmax} and by optimality of the set $S$, %of the states $s_\blj$ and $s_\blh$, 
%we have 
%\[\valj[\hat{s}] + \valh[\tilde{s}] = \valj[s_\blj] + \valh[s_\blh]\]
%Thus, Since $S$ is optimum for the state $s$, it follows that $S_\blj$ and $S_\blh$ are optimum for the states %$s_\blj$ and $s_\blh$, respectively. 
\end{proof}
%\end{comment}
\subsection{Bottom-Up Evaluation:Correctness of the DP Formulation}
\label{sec:bottomup}
\noindent {\bf Correctness invariant.} For a node $\bli$ and a valid state $s$ at $\bli$, the recursive definition in Section \ref{sec:recdef} ensures that
\[\soli[s] = \max_{\substack{D \subseteq V, |D| = k,\\ D\text{ induces }s}}\Ci(\Xi^+, D\cap \Xi^+)\] 
We prove this invariant by induction on the height of a node in the proof of the following theorem.
\begin{theorem}\label{theorem:fpt-by-wk}
The Uni-PBDS problem can be solved in time $2^{\Oh(w \log k)}n^2$ where $w$ is treewidth of the input graph.
\end{theorem}
%\begin{comment}
\begin{proof}
%We show that an optimal solution is obtained from the root $\blr$. 
  We first show that the bottom-up evaluation of the tables in $\TD$ maintains the correctness invariant.\\
{\em Claim:}
For each node $\bli$ in $\TD$, and for each state $s \in \Si$, the correctness invariant is maintained for $\soli[s]$.
\begin{proof}[Proof of claim]
The proof is by induction on the height of a node in $\TD$. Recall, that the height of a node $\bli$ in the rooted tree $\TD$ is the distance to the furthest leaf in the subtree rooted at $\bli$. 
The base case is when $\bli$ is a leaf node $\TD$ and height is 0 and the proof of the claim follows from Lemma ~\ref{lem:leaf}.
Let us assume that the claim is true for all nodes in $\TD$ of height at most $\ell-1 \geq 0$. 
We now prove that if the claim is true for all nodes of height at most $\ell-1$, then it is true for a node of height $\ell$. 
Let $\bli$ be a node of height $\ell \geq 1$. 
Since $\bli$ is not a leaf node,  its children are at height at most $\ell-1$. 
Therefore, by the induction hypothesis, the correctness invariant is maintained at all the chidlren of $\bli$.   %tables for the children are populated correctly by maintaining correctness invariant. 
Now, we prove that the correctness invariant is maintained at node $\bli$. Let $s$ be a state in node $\bli$.  
Let $S$ be an optimum solution at state $s$ in node $\bli$. We show that $\vali[s] = \Ci(\Xi^+,S)$. If $\bli$ is an introduce node then from  Lemma~\ref{lem:intr}, we know that the optimum coverage of $\Xj^+$ is achieved by $S \setminus \{v\}$ at state $s_\blj$ at node $\blj$.  Similarly, if $\bli$ is 
a forget node, then from Lemma ~\ref{lem:forget} we know that the optimum coverage of $\Xj^+$ is achieved by $S$ at state $s_\blj$ at node $\blj$. By the induction hypothesis in both these cases $\solj[s_\blj]$ is  the set which achieves optimum coverage, and this proves that  $\soli[s]$ is the optimum value at state $s$.  
 Further, if $\bli$ is a join node, then from the description of the computation at a join node, we know that $\vali[s]$ is recursively defined using $\vali[s_\blj]$ and $\vali[s_\blh]$ for an appropriate $s_\blj$ and $s_\blh$.  By the induction hypothesis, $\vali[s_\blj]$ and $\vali[s_\blh]$ are the optimal values. Therefore, it follows from Lemma ~\ref{lem:join} that $\C(\Xi^+,S) \leq \vali[s]$, and thus $\vali[s]$ is the optimum value.   
 %Tcan be written as the sum of $\C(\Xj^+,S)$, $\C(\Xh^+,S)$, with a term subtracted out which depends only on state $s$ at node $\bli$.  Further, Lemma ~\ref{lem:join} also shows that that $S$ induces the states $s_{\blj}$ and $s_{\blh}$ in the nodes $\blj$ and $\blh$, respectively.  
 Therefore, it  follows from the induction hypothesis that the solution and value are correctly computed at state $s$ based on the correct values computed at $s_\blj$ and $s_\blh$.   This completes the proof of the claim.
 \end{proof}
 \noindent
Finally, at the root node $\blr$, the state set $\S_\blr$ is a singleton set with a state $s = (k, \emptyset\to\{0,1\}, \emptyset\to[0,k], \emptyset \to [0,k])$.  By the induction hypothesis, the solution and the value maintained at this state are indeed the set that achieves the optimum coverage and the value of the coverage, respectively.
%We show that an optimal solution for the Uni-PBDS problem on instance $\langle \G, k \rangle$ is obtained from $\sol_\blr[s]$.
Finally, a node $\bli \in V(T)$ can have $k(2k+2)^{2w+3}$ states and each of them can be computed in time $\Oh((k+1)^{w+1}wn)$.
Since the nice tree decomposition $(T,X)$ has $\Oh(w\ n)$ nodes, the  tables at the nodes in $\TD$ can be computed in time $\Oh(w^2(2k+2)^{4w+8}n^2) = 2^{\Oh(w \log k)}n^3$.  This completes the proof of the theorem.
\end{proof}
%\end{comment}

